With Registered Reports Towards Large Scale Data Curation

The scale of manually validated data is currently limited by the effort that small groups of researchers can invest for the curation of such data. Within this paper, we propose the use of registered reports to scale the curation of manually validated data. The idea is inspired by the mechanical turk and replaces monetary payment with authorship of data set publication.

==> commands.tex <==
\newcommand{\etal}{~\textit{et al.}}
\newcommand{\AUC}{\textit{AUC}}
\newcommand{\FMEAS}{\textit{F-measure}}
\newcommand{\GMEAS}{\textit{G-measure}}
\newcommand{\MCC}{\textit{MCC}}
\newcommand{\AUCEC}{\textit{AUCEC}}
\newcommand{\RELB}{$RelB_{20\%}$}
\newcommand{\NECM}{$NECM_{15}$}
\newcommand{\RANKSCORE}{\textit{rankscore}}
\newcommand{\RANKSCORES}{\textit{rankscores}}
\newcommand{\RECALL}{\textit{recall}}
\newcommand{\PRECISION}{\textit{precision}}
\newcommand{\ERROR}{\textit{error}}

\newtheorem{definition}{Definition}%[section]
\newtheorem{notation}{Notation}%[section]
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corollary}{Corollary}
%\newtheorem*{proof}{Proof}%[chapter]
%\newcommand{\qed}{\hfill \ensuremath{\Box}}
